Security for Emerging Miniaturized Wireless Biomedical Devices: Threat Modeling with Application to Case Studies

The landscape of miniaturized wireless biomedical devices (MWBDs) is rapidly expanding as proactive mobile healthcare proliferates. MWBDs are diverse and include various injectable, ingestible, implantable, and wearable devices. While the growth of MWBDs increases the flexibility of medical services, the adoption of these technologies brings privacy and security risks for their users. MWBDs can operate with sensitive, private information and affect patients through the use of stimulation and drug delivery. Therefore, these devices require trust and need to be secure. Embedding protective mechanisms into MWBDs is challenging because they are restricted in size, power budget, as well as processing and storage capabilities. Nevertheless, MWBDs need to be at least minimally securable in the face of evolving threats. The main intent of this work is to make the primary stakeholders of MWBDs aware of associated risks and to help the architects and the manufacturers of MWBDs protect their emerging designs in a repeatable and structured manner. Making MWBDs securable begins with performing threat modeling. This paper introduces a domain-specific qualitative-quantitative threat model dedicated to MWBDs. The proposed model is then applied to representative case studies from each category of MWBDs.

==> sections/section_8.tex <==
\section{Bio-Sketches}
\label{sec:bio_sketches}

\textit{Vladimir Vakhter}: Vladimir Vakhter received his Specialist (a 5.5-year) degree (with honors) in Electronics and Automation of Physical Machines from the Ural Federal University (UrFU), Yekaterinburg, Russia in 2016. Being awarded by a Fulbright grant, he is currently pursuing his M.S. degree in Electrical and Computer Engineering at Worcester Polytechnic Institute (WPI), Worcester, Massachusetts, the U.S. For two and a half years, Vladimir conducted research of luminescent and scintillation materials at UrFU. Thereafter for two years, he developed a special magneto-optical system for the analysis of ferromagnetic materials at the Russian Academy of Sciences. Vladimir’s 3+ year professional experience includes working as an Electronics Engineer and as a Software Developer. Vladimir completed two short-term scientific internships in the Superconducting Quantum Circuits group at the Karlsruhe Institute of Technology (KIT), Karlsruhe, Germany in 2014 and 2015. His Master’s research at the Integrated Circuits and Systems Lab (ICAS) at WPI is focused on the security for wireless injectable, implantable, ingestible, and wearable resource-restricted biomedical devices.

\textit{Betul Soysal}: Betul Soysal received her B.Sc. (with honors) degree in Electrical and Electronics Engineering from Middle East Technical University, Turkey in 2006 and the M.S. degree from Bogazici University, Turkey  in 2010. She started her career as an IT Security Researcher in TUBITAK, the Scientific Research Council of Turkey. Betul was with TUBITAK from 2007 to 2016. She studied Cryptography, Embedded Device Security and ASIC Security; performed security evaluations for various product types, conducted side channel analysis and fault cryptanalysis for crypto devices and ICs; and performed threat modeling and risk analysis for large scale projects. Betul has been with Google since February 2019, focusing on Chromebook and Chrome OS security. Her research interests include run time user data security and she has special interest in resource-restricted biomedical devices and connecting with these devices securely.

\textit{Patrick Schaumont}: Patrick Schaumont is a Professor in Computer Engineering at WPI. He received the Ph.D. degree in Electrical Engineering from UCLA in 2004 and the MS degree in Computer Science from Ghent University in 1990. He was a staff researcher at IMEC, Belgium from 1992 to 2000. He was a graduate student and postdoc at UCLA from 2001 to 2005. He was a faculty member with Virginia Tech from 2005 to 2019. He joined WPI in 2020. He was a visiting researcher at the National Institute of Information and Telecommunications Technology (NICT), Japan in 2014. He was a visiting researcher at Laboratoire d'Informatique de Paris 6 in Paris, France in 2018. He is a Radboud Excellence Initiative Visiting Faculty with Radboud University, Netherlands from 2020. His research interests are in design and design methods of secure, efficient and real-time embedded computing systems. He served as program co-chair for several conferences in cryptographic and secure engineering, including CHES, HOST, ASHES, and FDTC. He received the National Science Foundation CAREER Award in 2007.

\textit{Ulkuhan Guler}:
Ulkuhan Guler received the B.Sc. degree in Electronics and Telecommunication Engineering from the Istanbul Technical University, Turkey, in 1999. She received the M.E degree in 2003, in Electronics Engineering from the University of Tokyo, Japan, and the Ph.D. degree in Bogazici University, Istanbul, Turkey, in 2014.
She joined the National Research Institute of Electronics & Cryptology, TUBITAK, Turkey, in 2006. Until 2015 summer, she was with the Semiconductor Technologies Research (YITAL) group in TUBITAK as a principal design engineer. She worked as a post-doc research fellow at Georgia Institute of Technology, from 2015 to 2018. In 2018, she joined the Department of Electrical and Computer Engineering, Worcester Polytechnic Institute, MA, where she is currently an Assistant Professor.
She studied security and cryptology, specifically oscillator-based True Random Number Generators (TRNG), during her Ph.D. In TUBITAK, her focus was on the design of smart cards and RFIDs,  including designing physical security sensors, random number generators (RNG), and security countermeasures on the chip level, as well as wireless power and data transmission, analog-front end circuits, and oscillators. During her studies at Georgia Institute of Technology, she focused on biomedical applications for healthcare technology development, while she was also working on energy harvesting, wireless power transmission, and power management for IoT and biomedical applications.
Dr. Guler’s research interests lie in the broad area of circuits and systems, and her primary area of interest is analog/mixed-signal integrated circuits.  Her interests for research include developing not only secure, smart, and connected technologies for healthcare applications but also general-purpose IoT applications. She served as a reviewer of various IEEE journals and conferences, as well as, as a technical committee member of several IEEE conferences including, CICC, BIOCAS, and MWSCAS. 


